SensiX++: Bringing MLOPs and Multi-tenant Model Serving to Sensory Edge Devices

We present SensiX++ - a multi-tenant runtime for adaptive model execution with integrated MLOps on edge devices, e.g., a camera, a microphone, or IoT sensors. SensiX++ operates on two fundamental principles - highly modular componentisation to externalise data operations with clear abstractions and document-centric manifestation for system-wide orchestration. First, a data coordinator manages the lifecycle of sensors and serves models with correct data through automated transformations. Next, a resource-aware model server executes multiple models in isolation through model abstraction, pipeline automation and feature sharing. An adaptive scheduler then orchestrates the best-effort executions of multiple models across heterogeneous accelerators, balancing latency and throughput. Finally, microservices with REST APIs serve synthesised model predictions, system statistics, and continuous deployment. Collectively, these components enable SensiX++ to serve multiple models efficiently with fine-grained control on edge devices while minimising data operation redundancy, managing data and device heterogeneity, reducing resource contention and removing manual MLOps. We benchmark SensiX++ with ten different vision and acoustics models across various multi-tenant configurations on different edge accelerators (Jetson AGX and Coral TPU) designed for sensory devices. We report on the overall throughput and quantified benefits of various automation components of SensiX++ and demonstrate its efficacy to significantly reduce operational complexity and lower the effort to deploy, upgrade, reconfigure and serve embedded models on edge devices.

==> sections/discussion.tex <==
\section{Discussion}

\textbf{Extension to multiple, distributed edges}

\textbf{Container-level optimisation:} adaptive docker construction, dynamic selection of model variants


\am{have a look at the comment here for some discussion on the data coordinator}
% \subsection{Data Coordinator Discussion}
% \begin{itemize}
%     \item Maybe at this level does not affect much the model throughput or overall system overhead because the transformations we apply to the data are quite simple (e.g. image re-scaling, drop frames, ...). One option to make this layer more `impactful' on the overall performance is if we consider more expensive operations like super-resolution, domain adaptation or similar. Another option is if the sensors are remote, in this case this layer should account for network issues (latency, drops, ...) which could significantly affect overall performance.
    
%     \item Maybe include this layer in the same section with the scheduler, not in a separate section, since this layer might be quite simple and not offer much contributions.
    
%     \item Is this problem still relevant if all HW manufacturers decide to standardise their sensors to offer `translation' capabilities directly on the sensors? R: It's very unlikely that device manufacturers will support all these transformations at the HW level, there will always be capabilities/requirements mismatches because typically sensors are build for specific use cases and offer only limited `transformations'. Think about 4k cameras used for surveillance and ultra-low power cameras used in batteryless sensors.
    
%     \item Limitations?
% \end{itemize}


\subsection{Model Creation Discussion}
Our design choice of creating docker containers on-the-fly during deployment is motivated by heterogeneity in the edge-ML ecosystem. In principle, model developers can also provide pre-built docker images to run their model; however since the installation of ML frameworks as well as numerical computing libraries differ across edge devices, this would require model developers to create device-specific variants of docker containers. \system\ abstracts this complexity by requiring developers to only provide the model weights and inference pipelines, and takes care of building device-specific docker images during deployment. 

Secondly, we made a choice of creating processor-specific containers and execution pipelines based on the current system load. While this design choice is apt for short-term inference requests (which are the primary use-case of \system\ ), it need not be optimal for long-term inference requests. For instance, the workload across processors may change significantly in minutes or hours, and our choice of processor may not remain optimal in the future. A possible solution to counter this challenge is to install all hardware-specific variants of a ML model (e.g., MobileNet-CPU, MobileNet-GPU, MobileNet-TPU) in the same or different docker containers and dynamically choose one of them based on system load. This solution however makes the system design and scheduler operations overly complex in a multi-model system, and adds additional latency associated with loading/unloading parameters into different processors' memory. Hence, we opt for a simpler system design in \system\ and propose that model containers can be rebuilt during system downtime to account for any changes in the system state.  


%%%%% OLD

\begin{comment}

\subsection{(Optional) Deployment Experience}

\textbf{Objective:} To show the benefit of "brining MLOps" aspect

\subsubsection{Application} \hfill

* Make a multi-tenant application scenario and show how it can be added to SensiX

* What to show? Example of model manifest file, logic functions
  - We can move code snippets in Section 4.5, here
  
 \utku{Model deployment latency? With and without the model already running on the system? }

\subsubsection{Operation} \hfill

* To show how the system operates with the same application on different hardwares (on AGX, Nano) \cm{different cameras as well?}

\utku{Is this really necessary? I think this goes without saying. AGX and nano have the same architecture. Only difference is that one is much stronger than the other. Besides, we use containers to provide a level isolation from the hardware.}

\pgfplotstableread[row sep=\\,col sep=&]{
    device & m1 & m2 & m3 \\
    agx & 100 & 98 & 95  \\
    nano & 74 & 75 & 77  \\
    }\devicedata
    
\begin{tikzpicture}
    \begin{axis}[
            ybar,
            symbolic x coords={agx,nano},
            xtick=data,
        ]
        \addplot table[x=device,y=m1]{\devicedata};
        \addplot table[x=device,y=m2]{\devicedata};
        \addplot table[x=device,y=m3]{\devicedata};
        \legend{$M_1$, $M_2$, $M_3$}
    \end{axis}
\end{tikzpicture}
 
\subsubsection{Deployment} \hfill

\cm{how about adding our SensiX demo interface 1) to show application can be simply added by pushing manifest/applet files, 2) to show example outputs}

\utku{I think that would just be distracting. }

\end{comment}


==> sections/interface.tex <==
% \subsection{System Interface Layer}
% SensiX interface layer serves both model/application developers, i.e. $2^\textrm{nd}$-party collaborators, and applications, $3^\textrm{rd}$-party users through REST APIs. These APIs allow developers to deploy their models and functions they use for application logic to interpret model outputs. Applications issue queries for model and function outputs using application facing APIs. In this section, we describe how SensiX handles model deployment and query processing in the interface layer.

\subsection{System Interface}
We provide a set of external APIs that allow developers to deploy their models and post-processing functions on the model output for application logic. Similarly, applications issue queries for model and function outputs using application facing APIs.
\subsubsection{Deployment}
\system\ provides a document-based deployment mechanism to model and application developers through an external POST API (\verb|/deploy|). This API accepts an archive of files to define the deployment. 

A \emph{manifest} file includes a list of descriptions for the models that a developer wants to deploy. This includes the name of the model, the framework it uses, a link to download the weights of the underlying neural network, etc. In addition, this file dictates the relationship of the model with other components. It dictates a description of the input data the model expects. %including the sensor type, e.g. camera, microphone; encoding, e.g. RGB, JPG, wav; size, e.g. 216x216 pixels, 5 seconds; sensor data freshness, etc.

A \emph{codelet} file provides executable functions that process the model output and provide an application logic. A \emph{functions} file on the other hand provides descriptions for these functions in the codelet. This includes the input t o each function, which can be outcome from one or more models and/or other functions.

These files then passed into the system components to create corresponding compute units and create a pipeline for end-to-end execution.

\subsubsection{Query Management}
\system can serve three types of queries. A \emph{one-off} query is issued when a result is needed just once, returning this result. A \emph{periodic} query prompts computation of a result continuously at a given interval, that is so large that a continuous connection is not necessary. This is answered with a response and a URL that can be used to retrieve the next result. A \emph{stream} query is similar to periodic however the rate at which a result captured is large enough to sustain the connection. In this case, the interface layer prepares a stream using the output of corresponding models or functions and serve the requester. \system components retrieves this execution rate and offers a best-effort mechanism to serve it. 

In order to limit redundant executions, the interface keeps these execution results in memory for a duration of interval specified in the query. This way identical queries that arrive consecutively responded quickly without requiring any interference. 

Query requests are issued to \system through application facing APIs. These APIs are summarized as below:
\begin{itemize}
\item \verb|/models|: Get the list of models
\item \verb|/functions|: Get the list of post-processing functions
\item \verb|/model/:model_id/:query_type|: Get the model output with a query type
\item \verb|/function/:function_id/:query_type|: Get the outcome of a post-processing function with a query type
\end{itemize}

==> sections/postprocessing.tex <==
\subsection{Post-Processing Functions\label{section:postprocessing}}
\system\ allows execution of post-processing functions that process the model outputs. These functions are serve a purpose to similar to \emph{serverless computing} functions where developers do not need to maintain their servers. When a request arrives, the serverless platform allocates the execution environment for a function to handle the request~\cite{amazon, ms, google}. It is also possible to chain together a number of such functions~\cite{akkus18sand}.

We dedicate a container for the execution of post-processing functions, which is prompted by query requests. \system\ allows model/application developers to add their functions to this container during deployment. This request sends a \emph{codelet} file to the post-processing container that provides a list of executable functions that uses the outcome from one or more other functions and/or models. The \emph{functions} file in the request on the other is used to create the chain of execution of several functions in sequence.

Consider two applications that use the outcome of an object recognition model whose outcome is a series of objects and their corresponding bounding boxes on the image used by the model. Assume one function counts the number of cars, and the other prepares an image where detected people are shown in bounding boxes. While the first function merely needs the model output, the second function needs the original image captured by the camera and the output of reshaping function applied on the model output to draw bounding boxes. A snippet for these functions is given in Figure~\ref{fig:codelet}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/codelet.png}
    \caption{A code snippet for functions in the codelet}
    \label{fig:codelet}
\end{figure}


